ShadowSense: Unsupervised Domain Adaptation and Feature Fusion for Shadow-Agnostic Tree Crown Detection from RGB-Thermal Drone Imagery

Accurate detection of individual tree crowns from remote sensing data poses a significant challenge due to the dense nature of forest canopy and the presence of diverse environmental variations, e.g., overlapping canopies, occlusions, and varying lighting conditions. Additionally, the lack of data for training robust models adds another limitation in effectively studying complex forest conditions. This paper presents a novel method for detecting shadowed tree crowns and provides a challenging dataset comprising roughly 50k paired RGB-thermal images to facilitate future research for illumination-invariant detection. The proposed method (ShadowSense) is entirely self-supervised, leveraging domain adversarial training without source domain annotations for feature extraction and foreground feature alignment for feature pyramid networks to adapt domain-invariant representations by focusing on visible foreground regions, respectively. It then fuses complementary information of both modalities to effectively improve upon the predictions of an RGB-trained detector and boost the overall accuracy. Extensive experiments demonstrate the superiority of the proposed method over both the baseline RGB-trained detector and state-of-the-art techniques that rely on unsupervised domain adaptation or early image fusion. Our code and data are available: https://github.com/rudrakshkapil/ShadowSense

==> resources/0_Revised_Tables.tex <==

% \newcommand*{\belowrulesepcolor}[1]{% 
%   \noalign{% 
%     \kern-\belowrulesep 
%     \begingroup 
%       \color{#1}% 
%       \hrule height\belowrulesep 
%     \endgroup 
%   }%
% } 
% \newcommand*{\aboverulesepcolor}[1]{% 
%   \noalign{% 
%     \begingroup 
%       \color{#1}% 
%       \hrule height\aboverulesep 
%     \endgroup 
%     \kern-\aboverulesep 
%   }%
% } 




\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}




\makeatletter
\def\igcite#1{%
     \begingroup
         \@fileswfalse
         #1%                     % do \cite comand
    \endgroup
}
\makeatother



\newcommand{\litReviewTable}{
\begin{table}[b]
\vspace{-0.15cm}
\centering
\caption{\textbf{Categorization of Related Works} according to training supervision through RGB ground truth (GT) annotations. 
% Asterisks ($^*$) indicate works we evaluated despite the lack of GT by omitting detection-specific losses, as described in \cref{sec:Experiments}. 
\label{tab:litReview}}
\vspace{-0.2cm}
{\small{
\renewcommand\arraystretch{1.25}
\resizebox{\columnwidth}{!}{
\begin{NiceTabular}{M{0.2\linewidth}|M{0.36\linewidth}|M{0.28\linewidth}}
    \toprule
    % \vspace{1cm}
    % \hline
    \cellcolor{white!20}\textbf{Category} & \cellcolor{red!20}{\textbf{GT Required}} & \cellcolor{green!20}{\textbf{GT Not Required}}\\%
    % \xmathstrut[0.5]{0} \\
    \midrule
    \midrule

    %%%% UDA
    UDA for Detection
    % GT NEEDED
    & 
    \cite{khodabandeh2019robust}
    \cite{Kieu2020}
    \cite{Lyu2022}
    \igcite{\cite{Mattolin2022}} 

    \igcite{\cite{Munir2021}} % contrastive
    \igcite{\cite{Pasqualino2021}} % DAT
    \igcite{\cite{Vidit2021}} % attention
    \cite{Vibashan2022} 
    
    \igcite{\cite{Yang2021}} 
    \igcite{\cite{Zhao2020}}
    \cite{Zheng2020}
    % GT NOT NEEDED
    & 
    \textbf{Ours}\\

    \cline{1-3}
    % \midrule

    %%% TRANSLATION
    RGB - Thermal Fusion
    % GT NEEDED - all SOD papers can be included here if needed, and text above changed to just RGB-Thermal Fusion. 
    & 
    \cite{Gao2022}
    \igcite{\cite{Liu2022a}}
    \cite{Liu2022}
    \igcite{\cite{Moradi2022}}
    \igcite{\cite{Zhao2023a}}
    

    % SOD:
    SOD:
    \igcite{\cite{Guo2021}}
    \igcite{\cite{Liao2022}}
    \igcite{\cite{Song2022}}
    
    \igcite{\cite{Tu2021}}
    \igcite{\cite{Wang2022}} 
    \igcite{\cite{Zhang2021}}
    \igcite{\cite{Zhou2022}}
    % GT NOT NEEDED
    & 
    \cite{Han2022}
    \igcite{\cite{Liu2022b}}

    \igcite{\cite{Wang2022a}}
    \igcite{\cite{Wang2023}} 
    \cite{Xu2022}
    
    and \textbf{Ours}\\

    \cline{1-3}
    %%% TRANSLATION
    Translation 
    % GT NEEDED
    & 
    \igcite{\cite{Chen2021}}
    \igcite{\cite{guo2023shadowformer}}
    % GET NOT NEEDED
    & 
    \igcite{\cite{Huang2018}}
    \igcite{\cite{Luo2022}}\\
    \bottomrule
\end{NiceTabular}}
% \vspace{-3.5mm}
}}
\end{table}
}


\newcommand{\datasetsTable}{
\begin{table}[t]
\centering
% \vspace{-0.2cm}
\caption{\textbf{Comparative Overview} of RGB-Thermal Image Datasets.} \label{tab:datasets}
\vspace{-0.2cm}
{\small{
\renewcommand\arraystretch{1.25}
\resizebox{\columnwidth}{!}{
\begin{NiceTabular}{l|c|c|c|c|c}
\toprule
\textbf{Dataset} & \textbf{\# Pairs} & \textbf{Dimensions} & \textbf{Year} & \textbf{GT} & \textbf{Application}\\
\midrule
\midrule
TNO \cite{Toet2022} & 63 & Various & 2014 & $\times$  & Image Fusion\\
MFNet \cite{Ha2017MFNetTR} & 1569 & 640$\times$480 & 2017 & \checkmark  & Semantic Segmentation\\
VIFB \cite{Zhang2020VIFBAV} &  21 &  Various & 2020 & $\times$  & Image Fusion \\
RoadScene \cite{Xu2020} & 221 & 768$\times$576 & 2020 & $\times$  & Image Fusion\\
LLVIP \cite{jia2021llvip} &  15488 & 1080$\times$720 & 2021 & \checkmark  & Pedestrian Detection\\
M$^3$FD \cite{Liu2022a} & 4200 & 1024$\times$768 & 2022 & \checkmark  & Object Detection\\
\textbf{RT-Trees (Ours)} &  49879 &  500$\times$500 & 2023 &  \checkmark (eval.)  & Tree Crown Detection \\
\bottomrule
\end{NiceTabular}}
}}
\vspace{-0.5cm}
\end{table}
}





\newcommand{\resultsTable}{
\begin{table*}[t]
\caption{\hl{\textbf{Quantitative Comparison}} of the proposed method with baseline and SOTA methods based on AP50 and AP100 metrics.
% Quantitative Results} showing Average Precision at 0.5 IoU (AP50), Average Recall with 100 predicted boxes (AR100) for various methods, and \% of shadowed trees identified. 
The best and second-best results are emboldened in \textcolor{red}{red (supervised)} and \textcolor{blue}{blue (self-supervised)}. \com{R_1C_{A5}, R_4C_6, R_5C_2} \label{tab:quant_results}}
\vspace{-0.2cm}
\centering
{\small{
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[0pt][0pt]}
\renewcommand\arraystretch{1.15}
\resizebox{0.9\linewidth}{!}{
\begin{NiceTabular}{p{3.35cm}p{0.15cm}|l|M{2.5cm}|cc|c}
    \toprule
    \multicolumn{2}{l}{\multirow{2}{*}{\thead{Evaluation}}}
    & \multirow{2}{*}{\thead{Method}}
    & \multirow{2}{*}{\thead{\hl{\centering Training Data}}}
    & \multicolumn{2}{c}{\thead{All Trees}}
    & \multicolumn{1}{c}{\thead{Shadowed Trees}} \\ \cmidrule{5-7}
    & & & & \thead{\hl{\%} AP50 $(\uparrow)$} & \thead{\hl{\%} AR100 $(\uparrow)$} & \thead{\% Identified $(\uparrow)$} \\%
    
    \midrule
    \midrule
    \multirow{4}{*}{\textbf{Baseline \cite{Weinstein2019}}}  
    & & 
    Off-The-Shelf Model (Eval. on RGB Images)
    & \multirow{2}{*}{\shortstack[c]{\parbox{\hsize}{\centering Pre-trained \\on NEON \cite{NEON}}}}
    & 49.86 %or .04 
    & 24.01 %or 23.44
    & 10.41 \\
    & & 
    Off-The-Shelf Model (Eval. on Thermal Images)
    & 
    & 4.34 & 2.27 & 2.82\\
    \cmidrule{3-7}
    & & 
    Supervised Fine-Tuned Model \hl{(Eval. on RGB Images)}
    & \multirow{2}{*}{\shortstack[c]{\parbox{\hsize}{\centering + Ann. RGB subset\\of RT-Trees}}}
    & \textbf{\textcolor{red}{55.20}} & \textbf{\textcolor{red}{29.42}} & \textbf{\textcolor{red}{20.10}} \\
    & & 
    \hl{Supervised Fine-Tuned Model (Eval. on Thermal Images)}
    & 
    &  5.64 &  3.98 & 3.81 \\

    \midrule
    \multirow{3}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Image Translation}\\Inference using \cite{Weinstein2019} \\on Generated Images}}}
    & & Increased Background Brightness in HSV Space
    & \centering N/A
    & 42.01 & 20.35 & 10.41 \\
    & & ShadowFormer \cite{guo2023shadowformer}: Shadow Removal 
    & \centering ISTD \cite{Wang2018_ISTD}
    & 11.62 & 6.48 & 3.47 \\
    & & PearlGAN \cite{Luo2022}: Thermal Image Colorization 
    & \centering RT-Trees
    & 40.72 & 19.67 & 11.18  \\
    
    \midrule
    \multirow{3}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Early Image Fusion}\\Inference using \cite{Weinstein2019} \\on Generated Images}}} 
    & & UMFusion \cite{Wang2022a}
    & \centering TNO \cite{Toet2022}
    & 38.00 & 18.56 & 10.20 \\
    & & MFEIF \cite{Liu2022b} 
    & \centering TNO \cite{Toet2022}
    & 39.62 & 18.95 & 15.40  \\
    & & MetaFusion \cite{Zhao2023a} 
    &\centering M$^3$FD \cite{Liu2022a}
    & 43.17 & 21.29 & 18.00 \\

    \midrule
    \multirow{8}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{RGB-Thermal\\ Unsupervised Domain\\ Adaptation (UDA) \hl{w/o\\Source Annotations}}\\Our Fused Inference \\after Adaptation}}}  
    & & SSTN \cite{Munir2021}: Contrastive Learning 
    & \centering RT-Trees
    & 31.53 & 15.16 & 2.13 \\
    & & Attention-based UDA \cite{Vidit2021} 
    & \centering RT-Trees & 31.97 & 15.34 & 3.84\\
    & & DA-RetinaNet \cite{Pasqualino2021}: ResNet DAT 
    & \centering RT-Trees &  32.88 & 15.72 & 3.65 \\ 
    \cmidrule{3-7}
    & \multirow{5}{*}{\rotatebox{90}{\textit{Ablation Study}}} 
    % & (i) \textbf{Ours}: FG FPN FA & 47.11 & 22.48 & 5.21  \\
    & $\>$$\-$ (i) \textbf{Ours}: FG FPN FA & \centering RT-Trees & 47.11 & 22.48 & 5.21  \\
    & & $\-$ (ii) \textbf{Ours}: ResNet DAT + FPN FA w/o Masking & \centering RT-Trees & 49.75 & 23.22 & 10.63 \\
    & & (iii) \textbf{Ours}: ResNet DAT + FG FPN FA (Pred. Masks) & \centering RT-Trees & 52.18 & 24.84 & 9.33 \\
    & & (iv) \textbf{Ours}: ResNet FG DAT + FG FPN FA & \centering RT-Trees & 52.24 & 24.38 & 14.32 \\
    & & $\-$ (v) \textbf{Ours} (\textbf{ShadowSense}): ResNet DAT + FG FPN FA & \centering RT-Trees & \textbf{\textcolor{blue}{54.13}} & \textbf{\textcolor{blue}{25.76}} & \textbf{\textcolor{blue}{19.09}} \\
    \bottomrule
\end{NiceTabular}}
}}
\vspace{-0.28cm}
\end{table*}
}




%% Ablation study. 
\newcommand{\ablationTable}{
\begin{table*}[!b]
\caption{\textbf{Extended Ablation Study} for different hyperparameter settings in the proposed method based on AP50 and AP100 metrics, trained without annotation on the RT-trees training set. Results on the RT-Trees validation set are reported. While changing one hyperparameter, all others are set to their best-performing values as described in the implementation details for the proposed ShadowSense configuration (also emboldened here).\label{tab:extended_ablation}}
\vspace{-0.2cm}
\centering
{\small{
\newcommand{\code}[1]{\texttt{##1}}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[0pt][0pt]}
\renewcommand\arraystretch{1.15}
\resizebox{0.95\linewidth}{!}{
% \resizebox{0.82\linewidth}{!}{
\begin{NiceTabular}{p{3.5cm}|l|cc|c}
    \toprule
    \multirow{2}{*}{\thead{Hyperparameter}}
    & \multirow{2}{*}{\thead{Value(s)}}
    & \multicolumn{2}{c}{\thead{All Trees}}
    & \multicolumn{1}{c}{\thead{Shadowed Trees}} \\ \cmidrule{3-5}
    & & \thead{\% AP50 $(\uparrow)$} & \thead{\% AR100 $(\uparrow)$} & \thead{\% Identified $(\uparrow)$}\\
    
    \midrule
    \midrule
    \multirow{7}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{FPN Alignment Scales $\beta$}\\In order of largest (lowest)\\ to smallest (highest) FPN level.}}}
    & 
    \code{[1.0, 1.0, 1.0, 1.0, 1.0]} Identical Weighting 
    & 54.02 & 24.73 & 19.20 \\
    &
    \code{[1.0, 1.0, 0.75, 0.5, 0.25]} Descending w/ Low Variance
    & 54.20 & 24.97 & 15.20 \\
    & 
    \textbf{\code{[1.0, 1.0, 0.5, 0.05, 0.01]}}{Descending w/ Med. Variance}
    & \textbf{55.48} & \textbf{25.86} & \textbf{20.80} \\
    & 
    \code{[1.0, 0.5, 0.1, 0.01, 0.005]} Descending w/ High Variance
    & 53.20 & 24.55 & 20.00 \\
    & 
    \code{[0.25, 0.5, 0.75, 1.0, 1.0]} Ascending w/ Low Variance
    & 50.96 & 24.70 & 12.80 \\
    & 
    \code{[0.01, 0.05, 0.5, 1.0, 1.0]} Ascending w/ Med. Variance
    & 50.21 & 24.61 & 13.60 \\   
    & 
    \code{[0.005, 0.01, 0.1, 0.5, 1.0]} Ascending w/ High Variance
    & 48.49 & 23.41 & 8.00 \\

    \midrule
    \multirow{7}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Fusion Scaling Weights $\eta$}\\In order of largest (lowest)\\ to smallest (highest) FPN level.}}}
    & 
    \code{[1.0, 1.0, 1.0, 1.0, 1.0]} Identical Weighting 
    & 54.62 & 24.28 & 19.60 \\
    &
    \code{[1.0, 1.0, 0.8, 0.6, 0.4]} Descending w/ Low Variance
    & 54.84 & 24.88 & \textbf{20.80} \\
    & 
    \textbf{\code{[1.0, 1.0, 0.5, 0.2, 0.2]}} {Descending w/ Med. Variance}
    & \textbf{55.48} & \textbf{25.86} & \textbf{20.80} \\
    &
    \code{[1.0, 0.5, 0.2, 0.05, 0.01]} Descending w/ High Variance
    & 51.71 & 23.00 & 20.00 \\
    & 
    \code{[0.4, 0.6, 0.8, 1.0, 1.0]} Ascending w/ Low Variance
    & 52.09 & 22.75 & 17.60 \\
    & 
    \code{[0.2, 0.2, 0.5, 1.0, 1.0]} Ascending w/ Med. Variance
    & 50.86 & 22.26 & 16.00 \\   
    & 
    \code{[0.01, 0.05, 0.2, 0.5, 1.0]} Ascending w/ High Variance
    & 48.81 & 21.07 & 10.40 \\

    
    \midrule
    \multirow{3}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Intensity Thresholds}\\Min. and max. markers\\used in mask generation.}}}
    & 
    \code{[30, 75]} Low number of initially unmarked intensities
    & 49.86 & 21.74 & 8.00 \\
    & 
    \textbf{\code{[20,100]}} {Medium number of initially unmarked intensities}
    & \textbf{55.48} & \textbf{25.86} & \textbf{20.80} \\
    &
    \code{[10,125]} High number of initially unmarked intensities
    & 51.67 & 22.23 & {18.40} \\
    
    
    \midrule
    \multirow{5}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Thermal Weight $\lambda_T$}\\Used in weighted fusion\\during inference.}}}
    &
    \code{0.5} Higher weighting for RGB features
    & 50.57 & 22.65 & 13.80 \\
    & 
    \code{1.0} Identical weighting for RGB and thermal features 
    & 50.31 & 22.03 & 16.00 \\
    &
    \code{2.5} \hspace{3.4mm}$|$
    & 52.61 & 23.08 & 18.40 \\
    & 
    \textbf{\code{5.0}} \hspace{3mm}$\downarrow$
    & \textbf{55.48} & \textbf{25.86} & \textbf{20.80} \\
    &
    \code{7.5} Higher weighting for thermal features
    & 52.01 & 22.86 & \textbf{20.80} \\

    \midrule
    \multirow{4}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Non-max Suppression}\\NMS threshold used in\\training and inference.}}}
    & 
    \code{0.05} Less overlap in filtered predictions
    & 49.15 & 22.25 & 17.20 \\
    &
    \code{0.10} \hspace{3.4mm}$|$
    & 50.50 & 23.30 & 16.00 \\
    & 
    \textbf{\code{0.15}} \hspace{3.0mm}$\downarrow$
    & \textbf{55.48} & \textbf{25.86} & \textbf{20.80} \\
    &
    \code{0.20} More overlap in filtered predictions
    & 50.60 & 23.97 & 17.20 \\

    
   

    \bottomrule
\end{NiceTabular}}
}}
\vspace{-0.28cm}
\end{table*}
}




%%

\newcommand{\datasetSplitTable}{
\begin{table*}[t]
\vspace{-0.15cm}
\centering
\caption{\textbf{RT-Trees Dataset Information by Flight Date}. All dates are from the year 2022. Information about the flight, lighting and weather conditions, and number of images is listed. Approximately 70\% of the raw image pairs captured for a given date are sampled for the training set based on GPS location (see \cref{fig:data}), and then divided into six 500$\times$500 patches. From the August 30 data, 63 images are taken for testing and 10 for validation, hence the total number of image pairs in RT-Trees is 49879. \label{tab:dataset_supplement_info}}
\vspace{-0.2cm}
{\small{
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[0pt][0pt]}
\renewcommand\arraystretch{1.25}
\resizebox{0.95\linewidth}{!}{
\begin{NiceTabular}{l|ccccc|cc}
    \toprule
    % \hline
    \thead{Flight Date} & \thead{Time of First \\Capture (24h)} & \thead{Flight \\Duration (min)} & \thead{Sun\\ Elevation ($^\circ$)} & \thead{Sun \\Azimuth ($^\circ$)} & \thead{Air \\Temperature ($^\circ C$)} & \thead{Raw Image \\Pairs Captured} & \thead{500$\times$500 Patches in\\ Training Set} \\%
    % \xmathstrut[0.5]{0} \\
    \midrule
    \midrule
    July 20      & 11:04 & 27 & 44.77 & 120.15 & 20.3 & 827 & 3582 \\
    July 26      & 10:18 & 28 & 37.51 & 109.32 & 20.8 & 828 & 3588 \\
    August 9     & 10:16 & 28 & 34.45 & 111.71 & 19.8 & 820 & 3552 \\
    August 17    & 12:15 & 33 & 46.12 & 147.29 & 24.5 & 825 & 3570 \\
    August 30    & 11:21 & 31 & 37.26 & 134.21 & 25.4 & 814 & 3516 \\
    September 9  & 11:40 & 32 & 36.08 & 142.39 & 14.0 & 824 & 3570 \\
    September 15 & 11:00 & 27 & 30.20 & 133.15 & 17.5 & 825 & 3582 \\
    September 23 & 11:14 & 28 & 29.12 & 139.04 & 14.7 & 820 & 3552 \\
    October 4    & 11:13 & 31 & 25.43 & 141.56 & 16.8 & 820 & 3558 \\
    October 6    & 15:16 & 27 & 27.22 & 210.10 &  9.8 & 808 & 3498 \\
    October 7    & 19:02 & 27 &  0.26 & 261.26 &  2.8 & 819 & 3552 \\
    October 12   & 10:53 & 27 & 20.92 & 138.40 & 11.5 & 826 & 3576 \\
    October 19   & 11:35 & 27 & 22.29 & 150.20 & 12.4 & 821 & 3558 \\
    November 24  & 16:10 & 28 &  2.21 & 230.46 &  4.7 & 819 & 3552 \\
    \midrule
    \thead{Total} & & & & & & \textbf{11496} & \textbf{49806} \\

    
    \bottomrule
\end{NiceTabular}}
% \vspace{-3.5mm}
}}
\end{table*}
}


==> resources/tables.tex <==

% \newcommand*{\belowrulesepcolor}[1]{% 
%   \noalign{% 
%     \kern-\belowrulesep 
%     \begingroup 
%       \color{#1}% 
%       \hrule height\belowrulesep 
%     \endgroup 
%   }%
% } 
% \newcommand*{\aboverulesepcolor}[1]{% 
%   \noalign{% 
%     \begingroup 
%       \color{#1}% 
%       \hrule height\aboverulesep 
%     \endgroup 
%     \kern-\aboverulesep 
%   }%
% } 


\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}




\makeatletter
\def\igcite#1{%
     \begingroup
         \@fileswfalse
         #1%                     % do \cite comand
    \endgroup
}
\makeatother



\newcommand{\litReviewTable}{
\begin{table}[b]
\vspace{-0.15cm}
\centering
\caption{\textbf{Categorization of Related Works} according to training supervision through RGB ground truth (GT) annotations. 
% Asterisks ($^*$) indicate works we evaluated despite the lack of GT by omitting detection-specific losses, as described in \cref{sec:Experiments}. 
\label{tab:litReview}}
\vspace{-0.2cm}
{\small{
\renewcommand\arraystretch{1.25}
\resizebox{\columnwidth}{!}{
\begin{NiceTabular}{M{0.2\linewidth}|M{0.36\linewidth}|M{0.28\linewidth}}
    \toprule
    % \vspace{1cm}
    % \hline
    \cellcolor{white!20}\textbf{Category} & \cellcolor{red!20}{\textbf{GT Required}} & \cellcolor{green!20}{\textbf{GT Not Required}}\\%
    % \xmathstrut[0.5]{0} \\
    \midrule
    \midrule

    %%%% UDA
    UDA for Detection
    % GT NEEDED
    & 
    \cite{Zheng2020}
    \cite{Kieu2020}
    \cite{Lyu2022}
    \cite{khodabandeh2019robust}

    \cite{Vibashan2021} 
    \igcite{\cite{Mattolin2022}} 
    \igcite{\cite{Zhao2020}}
    \igcite{\cite{Yang2021}} 
    
    
    \igcite{\cite{Vidit2021}} % attention
    \igcite{\cite{Pasqualino2021}} % DAT
    \igcite{\cite{Munir2021}} % contrastive
    % GT NOT NEEDED
    & 
    \textbf{Ours}\\

    \cline{1-3}
    % \midrule

    %%% TRANSLATION
    RGB - Thermal Fusion
    % GT NEEDED - all SOD papers can be included here if needed, and text above changed to just RGB-Thermal Fusion. 
    & 
    \igcite{\cite{Moradi2022}}
    \cite{Liu2022}
    \cite{Gao2022}
    \igcite{\cite{Liu2022a}}
    \igcite{\cite{Zhao2023a}}
    
    

    % SOD:
    SOD:
    \igcite{\cite{Wang2022}} 
    \igcite{\cite{Song2022}}
    \igcite{\cite{Zhou2022}}
    
    \igcite{\cite{Liao2022}}
    \igcite{\cite{Tu2021}}
    \igcite{\cite{Guo2021}}
    \igcite{\cite{Zhang2021}}
    % GT NOT NEEDED
    & 
    \cite{Han2022}
    \igcite{\cite{Wang2022a}}
    
    
    \cite{Xu2022}
    \igcite{\cite{Wang2023}} 
    \igcite{\cite{Liu2022b}}
    
    and \textbf{Ours}\\

    \cline{1-3}
    %%% TRANSLATION
    Translation 
    % GT NEEDED
    & 
    \igcite{\cite{Chen2021}}
    \igcite{\cite{guo2023shadowformer}}
    % GET NOT NEEDED
    & 
    \igcite{\cite{Luo2022}} \igcite{\cite{Huang2018}}\\
    \bottomrule
\end{NiceTabular}}
% \vspace{-3.5mm}
}}
\end{table}
}


\newcommand{\datasetsTable}{
\begin{table}[t]
\centering
\caption{\textbf{Comparative Overview} of RGB-Thermal Image Datasets.} \label{tab:datasets}
\vspace{-0.2cm}
{\small{
\renewcommand\arraystretch{1.25}
\resizebox{\columnwidth}{!}{
\begin{NiceTabular}{l|c|c|c|c|c}
\toprule
\textbf{Dataset} & \textbf{\# Pairs} & \textbf{Dimensions} & \textbf{Year} & \textbf{GT} & \textbf{Application}\\
\midrule
\midrule
TNO \cite{Toet2022} & 63 & Various & 2014 & $\times$  & Image Fusion\\
MFNet \cite{Ha2017MFNetTR} & 1569 & 640$\times$480 & 2017 & \checkmark  & Semantic Segmentation\\
VIFB \cite{Zhang2020VIFBAV} &  21 &  Various & 2020 & $\times$  & Image Fusion \\
RoadScene \cite{Xu2020} & 221 & 768$\times$576 & 2020 & $\times$  & Image Fusion\\
LLVIP \cite{jia2021llvip} &  15488 & 1080$\times$720 & 2021 & \checkmark  & Pedestrian Detection\\
M$^3$FD \cite{Liu2022a} & 4200 & 1024$\times$768 & 2022 & \checkmark  & Object Detection\\
\textbf{RT-Trees (Ours)} &  52869 &  500$\times$500 & 2023 &  \checkmark (eval.)  & Tree Crown Detection \\
\bottomrule
\end{NiceTabular}}
}}
\vspace{-0.5cm}
\end{table}
}






\newcommand{\resultsTable}{
\begin{table*}[t]
\caption{\textbf{Quantitative Comparison} of the proposed method with baseline and SOTA methods based on AP50 and AP100 metrics.
% Quantitative Results} showing Average Precision at 0.5 IoU (AP50), Average Recall with 100 predicted boxes (AR100) for various methods, and \% of shadowed trees identified. 
The best and second-best results are emboldened in \textcolor{red}{red} and \textcolor{blue}{blue}. \label{tab:quant_results}}
\vspace{-0.2cm}
\centering
{\small{
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[0pt][0pt]}
\renewcommand\arraystretch{1.15}
\resizebox{0.82\linewidth}{!}{
\begin{NiceTabular}{p{3.35cm}p{0.15cm}|l|cc|c}
    \toprule
    \multicolumn{2}{l}{\multirow{2}{*}{\thead{Evaluation}}}
    & \multirow{2}{*}{\thead{Method}}
    & \multicolumn{2}{c}{\thead{All Trees}}
    & \multicolumn{1}{c}{\thead{Shadowed Trees}} \\ \cmidrule{4-6}
    & & & \thead{AP50 $(\uparrow)$} & \thead{AR100 $(\uparrow)$} & \thead{\% Identified $(\uparrow)$} \\%
    
    \midrule
    \midrule
    \multirow{3}{*}{\textbf{Baseline \cite{Weinstein2019}}}  
    & & 
    Supervised Fine-Tuned Model
    % Supervised Fine-Tuning: RGB-only 
    & \textbf{\textcolor{red}{55.20}} & \textbf{\textcolor{red}{29.42}} & \textbf{\textcolor{red}{20.10}} \\
    & & 
    Off-The-Shelf Model on RGB Images
    % DeepForest \cite{Weinstein2019}: RGB-only 
    & 49.86 %or .04 
    & 24.01 %or 23.44
    & 10.41 \\
    & & 
    Off-The-Shelf Model on Thermal Images
    % DeepForest \cite{Weinstein2019}: Thermal-only 
    & 4.34 & 2.27 & 2.82\\

    \midrule
    \multirow{3}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Image Translation}\\Inference using \cite{Weinstein2019} \\on Generated Images}}}
    & & Increased Background Brightness in HSV Space & 42.01 & 20.35 & 10.41 \\
    & & ShadowFormer \cite{guo2023shadowformer}: Shadow Removal & 11.62 & 6.48 & 3.47 \\
    & & PearlGAN \cite{Luo2022}: Thermal Image Colorization & 40.72 & 19.67 & 11.18  \\
    
    \midrule
    \multirow{3}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Early Image Fusion}\\Inference using \cite{Weinstein2019} \\on Generated Images}}} 
    & & UMFusion \cite{Wang2022a}   & 38.00 & 18.56 & 10.20 \\
    & & MFEIF \cite{Liu2022b} & 39.62 & 18.95 & 15.40  \\
    & & MetaFusion \cite{Zhao2023a} & 43.17 & 21.29 & 18.00 \\

    \midrule
    \multirow{8}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Unsupervised Domain\\ Adaptation (UDA) w/o\\Source Annotations}\\Our Fused Inference \\after Adaptation}}}  
    & & SSTN \cite{Munir2021}: Contrastive Learning & 31.53 & 15.16 & 2.13 \\
    & & Attention-based UDA \cite{Vidit2021} & 31.97 & 15.34 & 3.84\\
    & & DA-RetinaNet \cite{Pasqualino2021}: ResNet DAT & 32.88 & 15.72 & 3.65 \\ \cmidrule{3-6}
    & \multirow{5}{*}{\rotatebox{90}{\textit{Ablation Study}}} 
    % & (i) \textbf{Ours}: FG FPN FA & 47.11 & 22.48 & 5.21  \\
    & $\>$$\-$ (i) \textbf{Ours}: FG FPN FA & 47.11 & 22.48 & 5.21  \\
    
    & & $\-$ (ii) \textbf{Ours}: ResNet DAT + FPN FA w/o Masking & 49.75 & 23.22 & 10.63 \\
    & & (iii) \textbf{Ours}: ResNet DAT + FG FPN FA (Pred. Masks) & 52.18 & 24.84 & 9.33 \\
    & & (iv) \textbf{Ours}: ResNet FG DAT + FG FPN FA & 52.24 & 24.38 & 14.32 \\
    & & $\-$ (v) \textbf{Ours} (\textbf{ShadowSense}): ResNet DAT + FG FPN FA & \textbf{\textcolor{blue}{54.13}} & \textbf{\textcolor{blue}{25.76}} & \textbf{\textcolor{blue}{19.09}} \\
    \bottomrule
\end{NiceTabular}}
}}
\vspace{-0.28cm}
\end{table*}
}



% \newcommand{\resultsTable}{
% \begin{table*}[t]
% \caption{\textbf{Quantitative Results} showing Average Precision (AP) and Average Recall with 100 predicted boxes (AR100) for various methods belonging to different groups of solutions. Best results are emboldened in red.}
% \begin{center}
% {\small{
% \renewcommand\theadfont{\bfseries}
% \renewcommand\theadgape{\Gape[0pt][0pt]}
% \renewcommand\arraystretch{1.15}
% \begin{NiceTabular}{p{3.5cm}|l||cc|cc}
%     \toprule
%     \multirow{2}{*}{\thead{Group}}
%     & \multirow{2}{*}{\thead{Method}}
%     & \multicolumn{2}{c}{\thead{All Trees}}
%     & \multicolumn{2}{c}{\thead{Shadowed Trees}} \\ \cmidrule{3-6}
%     & & \thead{AP $(\uparrow)$} & \thead{AR100 $(\uparrow)$} & \thead{AP $(\uparrow)$} & \thead{AR100 $(\uparrow)$} \\%
%     % \xmathstrut[0.5]{0} \\
    
%     \midrule
%     \multirow{3}{*}{\textbf{Baselines}} 
%     & Supervised Fine-Tuning: Thermal-only & ... & ... & ... & ... \\
%     & DeepForest \cite{}: RGB-only & ... & ... & ... & ... \\
%     & DeepForest \cite{}: Thermal-only & ... & ... & ... & ... \\

%     \midrule
%     \multirow{3}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Image Translation}\\DeepForest \cite{} Inference \\on Generated Images}}}
%     & ... & ... & ... & ... & ... \\
%     & ... & ... & ... & ... & ... \\
%     & ... & ... & ... & ... & ... \\

%     \midrule
%     \multirow{2}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Shadow Removal}\\DeepForest \cite{} Inference}}}
%     & Increase Background Brightness in HSV space & ... & ... & ... & ... \\
%     & ShadowFormer \cite{} & ... & ... & ... & ... \\
    
%     \midrule
%     \multirow{3}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Early Image Fusion}\\ DeepForest \cite{} Inference \\on Generated Images}}} 
%     & U2Fusion \cite{} & ... & ... & ... & ... \\
%     & PearlGAN \cite{} & ... & ... & ... & ... \\
%     & ICAFusion \cite{}   & ... & ... & ... & ... \\

%     \midrule
%     \multirow{5}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Domain Adaptation (DA) \\for RetinaNet}\\ Our Fused Inference \\after Adaptation}}}  
%     & &  ... & ... & ... & ... \\
%     & Thermal UDA Attention \cite{} & ... & ... & ... & ... \\
%     & DA-RetinaNet \cite{}: ResNet only & ... & ... & ... & ... \\ \cmidrule{2-6}
%     & \textbf{Ours}: DA for FPN only & ... & ... & ... & ... \\
%     & \textbf{Ours}: DA for ResNet and FPN & ... & ... & ... & ... \\
    
    
%     \bottomrule
% \end{NiceTabular}
% }}
% \end{center}
% \end{table*}
% }




% % \newcommand{\resultsTableOld}{
% % \begin{table*}[t]
% % \caption{\textbf{Quantitative Results} showing Average Precision (AP) and Average Recall with 100 predicted boxes (AR100) for different methods belonging to various groups of solutions. Best results are emboldened in red.}
% % \begin{center}
% % {\small{
% % \renewcommand\theadfont{\bfseries}
% % \renewcommand\theadgape{\Gape[0pt][0pt]}
% % \renewcommand\arraystretch{1.15}
% % \begin{tabular}{p{3.5cm}|l||cc|cc}
% %     \toprule
% %     \multirow{2}{*}{\thead{Group}}
% %     & \multirow{2}{*}{\thead{Method}}
% %     & \multicolumn{2}{c}{\thead{All Trees}} \vline
% %     & \multicolumn{2}{c}{\thead{Shadowed Trees}} \\ \cline{3-6}
% %     & & \thead{AP $(\uparrow)$} & \thead{AR100 $(\uparrow)$} & \thead{AP $(\uparrow)$} & \thead{AR100 $(\uparrow)$} \\%
% %     % \xmathstrut[0.5]{0} \\
    
% %     \midrule
% %     \multirow{3}{*}{\textbf{Baselines}} 
% %     & Supervised Fine-Tuning: Thermal-only & ... & ... & ... & ... \\
% %     & DeepForest \cite{}: RGB-only & ... & ... & ... & ... \\
% %     & DeepForest \cite{}: Thermal-only & ... & ... & ... & ... \\

% %     \midrule
% %     \multirow{3}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Image Translation}\\DeepForest \cite{} Inference \\on Generated Images}}}
% %     & ... & ... & ... & ... & ... \\
% %     & ... & ... & ... & ... & ... \\
% %     & ... & ... & ... & ... & ... \\

% %     \midrule
% %     \multirow{2}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Shadow Removal}\\DeepForest \cite{} Inference}}}
% %     & Increase Background Brightness in HSV space & ... & ... & ... & ... \\
% %     & ShadowFormer \cite{} & ... & ... & ... & ... \\
    
% %     \midrule
% %     \multirow{3}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Early Image Fusion}\\ DeepForest \cite{} Inference \\on Generated Images}}} 
% %     & U2Fusion \cite{} & ... & ... & ... & ... \\
% %     & PearlGAN \cite{} & ... & ... & ... & ... \\
% %     & ICAFusion \cite{}   & ... & ... & ... & ... \\

% %     \midrule
% %     \multirow{5}{*}{\shortstack[l]{\parbox{\hsize}{\textbf{Domain Adaptation (DA) \\for RetinaNet}\\ Our Fused Inference \\after Adaptation}}}  
% %     & &  ... & ... & ... & ... \\
% %     & Thermal UDA Attention \cite{} & ... & ... & ... & ... \\
% %     & DA-RetinaNet \cite{}: ResNet only & ... & ... & ... & ... \\ \cmidrule{2-6}
% %     & \textbf{Ours}: DA for FPN only & ... & ... & ... & ... \\
% %     & \textbf{Ours}: DA for ResNet and FPN & ... & ... & ... & ... \\
    
    
% %     \bottomrule
% % \end{tabular}
% % }}
% % \end{center}
% % \end{table*}
% }
